Self-Distilled Quantization: Achieving High Compression Rates in Transformer-Based Language Models

We investigate the effects of post-training quantization and quantization-aware training on the generalization of Transformer language models. We present a new method called self-distilled quantization (SDQ) that minimizes accumulative quantization errors and outperforms baselines. We apply SDQ to multilingual models XLM-R-Base and InfoXLM-Base and demonstrate that both models can be reduced from 32-bit floating point weights to 8-bit integer weights while maintaining a high level of performance on the XGLUE benchmark. Our results also highlight the challenges of quantizing multilingual models, which must generalize to languages they were not fine-tuned on.

==> figures/quant_by_layer_error_and_frobenius_norm_two_column.tex <==
\begin{figure*}[ht]
\centering
\begin{subfigure}{.445\textwidth}
  \centering
  \includegraphics[width=.975\linewidth]{images/quant_by_layer_type/xnli/quant_error_by_layer_type.png}
  \caption{Quantization Error}
  \label{fig:q_error}
\end{subfigure}%
\begin{subfigure}{.445\textwidth}
  \centering
  \includegraphics[width=.975\linewidth]{images/quant_by_layer_type/xnli/F_norm_diff_by_layer_type.png}
  \caption{F-Norm Elementwise Errors}
  \label{fig:f_norm}
\end{subfigure}
\vspace*{-1mm}
\caption{Dynamic Quantization of InfoXLM$_{\mathrm{Base}}$ After Quantization Aware Fine-Tuning on XNLI.}
\label{fig:xnli_qat_by_layer}
%\vspace*{-2mm}
\end{figure*}


==> sections/background.tex <==
\section{Background}
Quantization is the process of representing values with a reduced number of bits. In neural networks, this corresponds to weights, activations and gradient values. Typically, when training on a Graphics Processing Unit (GPU), values are stored in 32-bit floating point (FP) single precision. \textit{Half-precision} for floating point (FP-16) and integer arithmetic (INT-16) are also commonly considered. % INT-16 provides higher precision but a lower dynamic range compared to FP-16. In FP-16, the result of a multiplication is accumulated into a FP-32 followed by a down-conversion to return to FP-16. 
%
Previous work has focused on training and performing inference with lower-precision networks using integer precision (IP) as low as INT-8 INT-4, INT-2 or 1 bit representations~\citep{dally2015high} to speed up training and reduced inference time and bandwidth memory requirements.
% Designing such networks makes it easier to train such networks on CPUs, FPGAs, ASICs and GPUs. 
Two important features of quantization are the range of values that can be represented and the bit spacing. For the range of signed integers with $n$ bits, the range is $[-2n-1, 2n-2]$ and for full precision (FP-32) the range is $[-3.4 \times 1038, + 3.4 \times 1038]$. For signed integers, there are $2n$ values in that range and approximately $4.2 \times 109$ for FP-32. FP can represent a large array of distributions which is useful for neural network computation, however this comes at larger computational costs when compared to integer values. For integers to be used to represent weight matrices and activations, a FP scale factor is often used, hence many quantization approaches involve a hybrid of mostly integer formats with FP-32 scaling numbers, as in \emph{this work}. This is referred to as mixed-precision (MP) and different MP strategies have been used to avoid overflows during training and/or inference of low resolution networks given the limited range of integer formats. 
%
In practice, this often requires the storage of hidden layer outputs with full-precision (or at least represented with more bits than the lower resolution copies). The main forward-pass and backpropogation is carried out with lower resolution copies and converted back to the full-precision stored ``accumulators'' for the gradient updates. 

QAT aims to quantize the model during training~\cite{banner2018scalable,chmiel2020neural,faghri2020adaptive,kim2020position,wang2018training}. QAT is particularly useful as the number of bits reduces as training (or retraining) with methods that enable a neural network to be robust to quantization noise becomes increasingly important to maintain performance. For example, quantizing from FP-32 to INT-8 (or lower) with no QAT can result in an undesired drop in performance. Retraining quantized networks has been effectively used to maintain accuracy~\citep{gysel2018ristretto} in such cases and is referred to as iterative quantization (iQ). One effective approach to iQ is iterative product quantization (iPQ)~\cite{stock2019and} which uses vector quantization to generate a low-memory codebook by decomposing the subvectors of the weight matrices separately. We discuss current SoTA approaches to QAT in the next section that also build on iPQ. 

==> sections/experimental_setup.tex <==
\section{Experimental Setup}
Below describes the experimental details, including model, hyperparameter and quantization details.
\subsection{Model and Hyperparameters Details}
We choose modestly sized cross-lingual language models as the basis of our experiments, namely XLM-R$_{\text{base}}$~\cite{conneau2019unsupervised} and InfoXLM$_{\text{base}}$~\cite{chi2020infoxlm}. This is motivated by previous and expected findings that larger overparameterized networks suffer less from PTQ to 8-bit integer format and lower\citep{jacob2018quantization,krishnamoorthi2018quantizing}. Hence, to give a clear idea of how much compression can be achieved we make it more difficult as the models are already relatively small and are required to generalized to languages other than the language used for fine-tuning. 
For both XLM-R$_{\text{base}}$ and InfoXLM$_{\text{base}}$ the hyper-parameters are set as follows: 768 hidden units, 12 heads, GELU activation, a dropout rate of 0.1, 512 max input length, 12 layers in encoder. The Adam Optimizer with a linear warm-up~\cite{vaswani2017attention} and set the learning rate to 2e-5 for most tasks. For all sentence classification tasks the batch size is set to 32 and we fine-tune with 10 epochs. For POS Tagging and NER, we fine-tune with 20 epochs and set the learning rate to 2e-5. We select the model with the best average results on the development sets of all languages. For SDQ-based models, we report the best performing model for $\alpha \in [0.1, 0.2, 0.5, 0.8]$ and $\beta \in [10, 100, 200, 500]$. All experiments are carried out on Tesla V100-SXM2 32 Gigabyte GPUs~\cite{nvidia2017nvidia}.

% For MLQA, we set the learning rate to 3e-5, batch size to 12 and train 2 epochs following BERT for SQuAD. After each epoch, we test the fine-tuned model on the dev sets of all languages. We select the model with the best average result on the dev sets of all languages.

\subsection{Quantization Details. }%\mbox{}\\
For XGLUE tasks, XLM-RoBERTA$_{\mathrm{Base}}$ and InfoXLM$_{\mathrm{Base}}$ are quantized. We primarily focus on quantizing FP-32 networks to INT-8 networks but also include an analysis of the effects of quantization for varying bit ranges. %For static quantization methods that require calibration data to estimate the quantization bins of activations, we use the training data the model is fine-tuned on for minmax calibration. 
For all quantization methods, the input embedding layers and the classification layer are not quantized. We found quantizing either of these layers drastically reduces performance for all tasks. 
We denote QuantNoise based QAT training as QNAT and thus if used with we subscript the distillation loss to indicate this e.g QNAT$_{\text{Att-KLD}}$ use QuantNoise with the two distillation losses described in~\autoref{eq:sdq_loss}. For inference, we perform PTQ because in practice QAT applies \textit{fake} quantization and hence our reported results are after \emph{real} quantization using the ONNX Runtime~\cite{onnxruntime}. 

\iffalse
\begin{itemize}
\item \textbf{Dynamic Quantization} - 
\item \textbf{Static Quantization} - Quantizes both weights and activations, estimating activation quantization bins using a dataset for calibration.
\begin{itemize}
    \item Min-max quantization
    \item Entropy quantization
    \item Percentile quantization
\end{itemize}
\item Quantization Aware-Training
\begin{itemize}
    \item Quant-Noise
    \item Huffman Coding 
\end{itemize}
    \item \textbf{D}
\end{itemize}
\fi

\iffalse
\begin{figure}
    \centering
    \includegraphics[scale=0.5]{images/xglue/quant_by_layer_type/xnli/quant_error_by_layer_type.png}
    \caption{\textbf{Dynamic Quantization of InfoXLM$_{\mathrm{Base}}$ After Quantization Aware Fine-Tuning on XNLI}}
    \label{fig:quant_by_layer_type}
\end{figure}
\fi


==> sections/methodology.tex <==
\section{Methodology}
We begin by defining a dataset $\mathcal{D}: = \{(X_i, y_i)\}^D_{i=1}$ with single samples $s_i = (X_i, \vec{y}_i)$, where each $X_i$ (in the $D$ training samples) consists of a sequence of vectors $X_i := (\vec{x}_1, \ldots, \vec{x}_N)$ and $\vec{x}_i \in \mathbb{R}^{d}$. For structured prediction (e.g., NER, POS) $y_i \in \{0, 1\}^{N \times d_y}$, and for single and pairwise sentence classification, $y_i \in \{0, 1\}^{d_y}$, where $d_y$ is the number of classes.
%
Let $\vec{y}^S=f_{\theta}(X_i)$ be the output prediction ($y^{S} \in \mathbb{R}^{d_y}$) from the student $f_{\theta}(\cdot)$ with pretrained parameters $\theta:= \{\mat{W}_l, \vec{b}_l\}_{l=1}^{L}$ for $L$ layers. The input to each subsequent layer is denoted as $\vec{z}_{l} \in \mathbb{R}^{n_{l}}$ where $ \vec{z}_0 \coloneqq \vec{x}$ for $n_l$ number of units in layer $l$ and the corresponding output activation as $\vec{A}_{l} = g(\vec{z}_{l})$. 
%
The loss function for standard classification fine-tuning is defined as the cross-entropy loss $\ell_{CE}(\vec{y}^S, \vec{y}):= -\frac{1}{d_y}\sum_{i=1}^{d_y} \vec{y}_{d_y}\log(\vec{y}^s_{d_y})$.% where for a single sample $s_i$, $\mathcal{L}: \mathcal{Y} \times \mathbb{R}^n \to \mathbb{R}$. 

% When $m$ is set to $1$, PQ is equivalent to vector quantization (VQ) and when $m$ is equal to $C_{in}$, it is the scalar k-means algorithm. 

%The main benefit of PQ is its expressivity: each column $w_j$ is mapped to a vector in the product $C = C \times \cdots \times C$, thus PQ generates an implicit codebook of size $k_m$.

\subsection{Self-Distilled Quantization}
For self-distilled quantization, we also require a fine-tuned teacher network $f_{\Theta}$, that has been tuned from the pretrained state $f_{\theta}$, to retrieve the soft teacher labels $y^{T} := f_{\Theta}(\vec{x})$, where $y^{T} \in \mathbb{R}^C$ and $\sum_c^C y^{T}_c=1$. The soft label $\vec{y}^{T}$ can be more informative than the one-hot targets $\vec{y}$ used for standard classification as they implicitly approximate pairwise class similarities through logit probabilities.
% After fine-tuning $f_{\theta}$ through stochastic gradient descent (SGD), the output activations of $f_{\Theta}$ are used to perform self-distillation.
The Kullbeck-Leibler divergence (KLD) $\ell_{\mathrm{KLD}}$ is then used with the main task cross-entropy loss $\ell_{CE}$ to express $\ell_{\mathrm{SDQ}_{\text{KLD}}}$ as shown in \autoref{eq:sdq_loss}, 
%
\begin{equation}
\begin{split}\label{eq:kld_loss}
\ell_{\mathrm{SDQ}_{\text{KLD}}} \text{=}\, \ell_{\mathrm{CE}}(\vec{y}^{S}, \vec{y})\text{+}
\alpha \tau^2 D_{\mathrm{KLD}}\big(\vec{y}^{S}, \vec{y}^{T}\big)   
\end{split}    
\end{equation}


where $D_{\mathrm{KLD}}(\vec{y}^{S},\vec{y}^{T}) = \mathbb{H}( \vec{y}^T) - \vec{y}^{T} \log(\vec{y}^{S})$, $\mathbb{H}(\vec{y}^T)=\vec{y}^{T}\log(\vec{y}^{T})$ is the entropy of the teacher distribution and $\tau$ is the softmax temperature. Following~\cite{hinton2015distilling}, the weighted sum of the cross-entropy loss and the KLD loss shown in \autoref{eq:sdq_loss} is used as our main SDQ-based KD loss baseline, where $\alpha \in [0, 1]$. However, $D_{\mathrm{KLD}}$ only distils the knowledge from the soft targets which may not propagate enough information about the intermediate dynamics of the teacher. 
This brings us to our proposed attention-based SDQ loss $\ell_{\mathrm{SDQ}_{\text{Att-KLD}}}$ shown in~\autoref{eq:sdq_loss},
\begin{equation}
\begin{split}\label{eq:sdq_loss}
\ell_{\mathrm{SDQ}_{\text{Att-KLD}}} \text{=} \ell_{\mathrm{CE}}(\vec{y}^{S}, \vec{y}) \text{+}
\alpha \tau^2 D_{\mathrm{KLD}}\big(\vec{y}^{S}, \vec{y}^{T}\big) \\ 
+\beta \frac{1}{LH}\sum_{l=1}^{L}\sum_{h=1}^{H}\ell_{\mathrm{Attention}}\big(\mat{A}^{S}_{lh},\mat{A}^{T}_{lh}\big)  
\end{split}    
\end{equation}
where $\alpha$ and $\beta$ are regularization terms and $\ell_{\text{Attention}}$ computes the loss between the student and teacher outputs of each self-attention block in $L$ layers and $H$ attention heads per layer. We also consider two baselines, $\ell_{\text{SDQ}_\text{Att}}$ which is the same as~\autoref{eq:sdq_loss} without $\alpha \tau^2 D_{\mathrm{KLD}}(\vec{y}^{S}, \vec{y}^{T})$ and $\ell_{\text{SDQ}_\text{Hid}}$ which applies the Mean Squared Error (MSE) loss between the hidden state outputs instead of the attention outputs. The gradient of $D_{\text{KLD}}(\cdot,\cdot)$ is expressed as $\frac{\partial D_{\text{KLD}}(\vec{y}^{S}_i, \vec{y}^{T}_i)}{\partial \vec{y}^S_i} = \tau(\vec{y}^S_i/\tau - \vec{y}^T_i/\tau)$ and as $\tau \to \infty$, the gradient is approximately $1/d_y(\vec{y}^S_i - \vec{y}^T_i)$. Similarly, the gradient of the MSE loss on a single self-attention output in layer $l$ and head $h$ is $1/n_{lh}(\vec{a}^S_j - \vec{a}^T_j)$ for a single sample input $x$. Hence, we see the connection between derivatives between the KLD loss and the MSE loss when combining them in a single objective. We now move to desribing how SDQ is used in two QAT methods. 

\iffalse
We can then expressed the gradient step as,

\begin{equation}\label{eq:grad}
\begin{split}
    \mat{W}_{(t+1)} := \mat{W}_t - \eta \mathbb{E}_{
(X,y)\sim \mathcal{D}}(\tau(\vec{y}^S/\tau - \vec{y}^T/\tau) \\
+ (\mat{a}^S-\mat{a}^T)) - \nabla_{\mat{W}_t}\vec{y}^S
\end{split}
\end{equation}
\fi

%
\iffalse
Note that \emph{scaled} dot-product is used (normalization by $\sqrt{d_k}$) to avoid vanishing gradients of the $\mathrm{Softmax}$, which may occur when $d_k$ is large. 

The parameters for the $j$-th attention head $\mat{K}^j, \mat{V}^j \in \mathbb{R}^{d \times l}$, $\mat{U}^j \in \mathbb{R}^o$ for $j = 1,\ldots, n_a$ where $n_a$ is the number of attention heads. Then we summarize the formulation of multi-headed self-attention as Equation \eqref{eq:multi_head_att},
%
\begin{equation}\label{eq:multi_head_att}
\begin{split}
\mat{Z}^j & = \text{Softmax}\Big(\frac{\mat{Q}\mat{K}^j}{\sqrt{d_k}}(\mat{V}^j)^{\top}\mat{Q}^{T}\Big)\mat{Q}\mat{U}^j \\
\tilde{\mat{Z}} & = \mathrm{Concat}(\mat{Z}^1, \ldots \mat{Z}^n_a) \\
\mat{Z} & = \mathrm{Feedforward}(\mathrm{LayerNorm}(\tilde{\mat{Z}} + \mat{Q}))    
\end{split}
\end{equation}
%
where $\mat{Z}^{j} \in \mathbb{R}^{n \times d_{a}}$ and $\tilde{\mat{Z}} \in \mathbb{R}^{n \times d_{a}n_{a}}$, with $d_{a}$ being the dimensionality of the self-attention output.
\fi
\subsection{Iterative Product Distilled Quantization}
We first consider using SDQ with iPQ~\cite{stock2019and}. This is achieved by quantizing $m$ subvectors for each $k$ columns of $\mat{W}$ where a codebook for each $k$ subvectors is learned to map each subvector to its nearest neighbor in the learned codebook $C \in \mathbb{R}^{k\times d}$ where $k$ is the number of codewords. Any column $\mat{W}_{[:,i]}$ is mapped to its quantized version $\phi(\mat{W}_{[:,i]}) = (C_{[j,1]} \ldots, C_{[j,m]})$ where $[i,1]$ denotes the index of the codeword assigned to the first subvector of $\mat{W}_{[:,j]}$. The codebook is updated by minimizing,
\begin{equation}
||\mat{W} - \tilde{\mat{W}}||_2^2 = \sum_i^d || \mat{W}_{[:, i]} - \phi(\mat{w}_{[:, i]})||^2_2
\end{equation}
where $\phi(\cdot)$ is the quantization function. This objective can be efficiently minimized with the k-means algorithm and the codewords of each layers are updated with SGD by averaging the gradients of each assigned block of weights. This is done iteratively from the bottom layers to the top layers throughout training where the upper layers are finetuned while the lower layers are progressively being quantized~\cite{stock2019and}. When using iPQ with SDQ, omitting the KLD loss and cross-entropy loss, we can describe the objective as,
\begin{equation}
    \ell_{\text{SDQ}_{\text{iPQ}}} =\sum_{l=1}^{L-F}\Big[||\mat{W}_l - \tilde{\mat{W}}_l||^2_2 + \frac{\beta}{L\text{-}F}\sum_i^d(\mat{A}^{S}_{l,i} - \mat{A}^T_{l,i})^2\Big]
\end{equation}
where $F$ is the number of finetuned layers (non-quantized) at that point in training. Hence, SDQ is also iterative in this context and becomes more dominant as the network progressively becomes more quantized.

\subsection{Block-Wise Distilled Quantization Noise}
For the majority of our QAT-based experiments we use Quant-Noise~\cite{fan2020training}. Quant-Noise is a SoTA QAT method that applies (fake) block-wise quantization noise at random to each weight matrix. Concretely, blocks of weights $b_{kl}$ in $\mat{W}_l$ are chosen at random at a rate $p$ and quantization noise is added to the chosen blocks. 
%
For describing the use of SDQ-based QuantNoise in Transformers, we begin by defining $\mat{W}_Q \in \mathbb{R}^{n \times d}$ to be a matrix representing the sequence where the i-th row of $\mat{W}_Q$ corresponds to $\vec{x}_i$. The key $\mat{W}_K \in \mathbb{R}^{d \times l}$, value $\mat{W}_V \in \mathbb{R}^{d \times l}$ and projection layer $\mat{W}_U \in \mathbb{R}^{d \times o}$ parameters are defined where $\mat{U}$ ensures the output dimensionality of the self-attention block is identical to the original input $\mat{W}_Q$. We then define the self-attention as Equation \eqref{eq:self_att_1},
%
\begin{equation}\label{eq:self_att_1}
\mat{A}^T = \text{Softmax}\Big(\frac{\mat{W}_Q\mat{W}_K}{\sqrt{d_k}}\mat{W}^{\top}_V\mat{W}^{\top}_Q\Big)\mat{W}_Q\mat{W}_U    
\end{equation}
where $\mat{Q}\mat{U} \in \mathbb{R}^{n \times o}$ is matrix of new embeddings, $\mat{W}_Q\mat{W}_K\mat{W}^{\top}_V\mat{W}^{\top}_Q \in \mathbb{R}^{n \times n}$ is a matrix representing the inner products in a new $l$-dimensional space and $\mathrm{Softmax}\big(\mat{W}_Q\mat{W}_K\mat{W}^{\top}_V\mat{W}^{\top}_Q\big)$ is a matrix where each row entry is positive and sums to 1 and the $\sqrt{d_k}$, the embedding dimension, normalizes the input to avoid vanishing gradients of the $\mathrm{Softmax}$. 
We then define $\mat{A}^S = \text{Softmax}\big(\frac{\tilde{\mat{W}}_Q\tilde{\mat{W}}_K}{\sqrt{d_k}}\tilde{\mat{W}}^{\top}_V\tilde{\mat{W}}^{\top}_Q\big)\tilde{\mat{W}}_Q\tilde{\mat{W}}_U$ where $\tilde{\mat{W}}$ represents (fake) quantized weights and is given as,

\begin{equation}
\tilde{\mat{W}} = \phi_{\text{INT-8}}(\mat{W}) = s(\mathrm{round}(\mat{W}/s + b) - b)
\end{equation}
where $s$ and $b$ are scalars learned throughout training and represent the scaling factor and offset respectively. We can than pass $\mat{A}^S$ and $\mat{A}^T$ to~\autoref{eq:sdq_loss} to compute the loss.
%
Algorithm \ref{alg:sdq} illustrates the proposed framework of SDQ with QuantNoise (SDQ$_{\text{Att-KLD}}$) in $\mathrm{PyTorch}$ pseudocode used for sentence classification.  In this code $\mathrm{student\_model}$ contains forward hooks that apply $\mathrm{QuantNoise}$.
% We now move to describing the experimental setup before discussing the experimental results. 

\begin{figure}
\begin{minipage}{0.5\textwidth}
\begin{algorithm}[H]
   \caption{PyTorch pseudo-code of SDQ.}
   \label{alg:sdq}
   
    \definecolor{codeblue}{rgb}{0.25,0.5,0.5}
    \lstset{
      basicstyle=\fontsize{7.2pt}{7.2pt}\ttfamily\bfseries,
      commentstyle=\fontsize{7.2pt}{7.2pt}\color{codeblue},
      keywordstyle=\fontsize{7.2pt}{7.2pt},
    }
\begin{lstlisting}[language=python]
# model: student Transformer 
# teacher_model: fine-tuned Transformer
# alpha, beta: distillation loss weights
# method: chosen pruning criteria 
# prune_rate: compression amount in [0, 1] 
# lambda: weight on the off-diagonal terms
for x in loader: # batch loader of N samples
    # input_ids,attention_id & label_ids.
    x = tuple(xs.to(device) for xs in x)
    inputs = {"input_ids": x[0],
    "attention_mask": x[1], "labels": x[2]}
    outputs = student_model(**inputs)
    teacher_outs = teacher_model(**inputs)
    distil_loss = F.kld_divergence_loss(
        x[2], teacher_outs[2])
    # inputs last hidden representation for
    # [CLS] token and applies Equation 2. 
    attention_loss = 0
    for att_out, teacher_att_out in zip(outputs[1][-1], teacher_outs[1][-1]): 
        attention_loss += mse_loss(att_out,
        teacher_att_out, lambda)
    # loss given as first element in tuple    
    loss = outputs[0] + alpha * kld_loss 
    + beta * attention_loss  
    # compute backprop and update gradients
    loss.backward()
    optimizer.step()
# apply dynamic quantization after training
quant_model = quantize_model(model)
\end{lstlisting}
\end{algorithm}
\end{minipage}
\end{figure}
